The super-LHC

We review here the prospects of a long-term upgrade programme for the Large Hadron Collider (LHC), CERN laboratory's new proton-proton collider. The super-LHC, which is currently under evaluation and design, is expected to deliver of the order of ten times the statistics of the LHC. In addition to a non-technical summary of the principal physics arguments for the upgrade, I present a pedagogical introduction to the technological challenges on the accelerator and experimental fronts, and a review of the current status of the planning.

==> Makefile <==
# -*- makefile -*-
TARGETNAME=slhc-hepph

TEXFILES= $(TARGETNAME).tex tCPH2e.cls

PDFFILES= H-susy-reach.pdf Zpmodels.pdf Zpreach.pdf cerncomplex.pdf\
complexupgrade.pdf coupl1.pdf coupl2.pdf crabcrossing.pdf\
crossingangle.pdf jets.pdf lum33.pdf lum35.pdf lumprofile.pdf\
lumprofile_lev.pdf lumupgrade.pdf multiH.pdf pileup.pdf pileup_lev.pdf\
susy.pdf susyFS.pdf wz1.pdf wz2.pdf

#EPSFILES= 

#cluana.eps 
GZ=$(patsubst %.eps,%.gz,$(VEPS))
EPS=$(patsubst %.fx,%.eps,$(FXFILES)) $(patsubst %.top,%.eps,$(TOPFILES)) \
    $(patsubst %.eps.gz,%.eps,$(SEPS))
PDF= $(PDFFILES)
#$(patsubst %.eps,%.pdf,$(EPSFILES))
FILES= Makefile \
       $(TEXFILES) $(PDFFILES)

GZFILES= $(FILES) $(TARGETNAME).pdf
## user makefile has following lines
#include Makefile.$(shell uname)
#TARGETNAME=bbcorr96
#TEXFILES=files.tex ...
#FXFILES=files.fx ...
#TOPFILES=files.top ...
#EXTRAS=hep-ph.txt hep-ph.9607347 etc.
#EPS=$(patsubst %.fx,%.eps,$(FXFILES)) $(patsubst %.top,%.eps,$(TOPFILES)) 
#FILES= Makefile Makefile.AIX Makefile.Linux Makefile.SunOS \
#       $(TEXFILES) $(TOPFILES) $(FXFILES) $(EXTRAS)
#
#

# Standard tex Makefile, P. Nason, 6-8-96

#%.gz: %.eps
#	cp $*.eps ../plots/seps/$*.eps
#	gzip -9 ../plots/seps/$*.eps

#%.eps: %.fx
#	echo $* ~nason/scripts/nfeynx/ps-fonts | ~nason/scripts/nfeynx
%.pdf: %.eps
	epstopdf $*.eps

pdf: $(TARGETNAME).pdf

$(TARGETNAME).pdf:  $(TARGETNAME).tex $(EPS) $(PDF)
	if pdflatex $(TARGETNAME).tex ; then \
          if grep "Rerun to get cross-references right" $(TARGETNAME).log ; \
           then pdflatex $(TARGETNAME).tex ; fi ; \
           if grep "Rerun to get cross-references right" $(TARGETNAME).log ; \
           then pdflatex $(TARGETNAME).tex ; fi ; \
            fi
#	pdflatex $(TARGETNAME).tex

tgz: $(TARGETNAME).tgz

$(TARGETNAME).tgz: $(GZFILES)
	excluded=`for i in * ; do echo $(GZFILES) | grep -q $$i ; \
          if [ $$? != 0 ] ; then echo $$i ; fi ; done` ; \
          if [ "z$$excluded"!=z ] ; then echo " " ; \
          echo 'Excluded files:' $$excluded ; echo " " ; fi
	tar zcvf $(TARGETNAME).tgz $(GZFILES)

clean:
	-rm *~ *.log *.dvi *.aux *.toc *.uu *.o a.out core log

epsclean:
	-rm *.eps



